(Optimal) Online Bipartite Matching with Degree Information

We propose a model for online graph problems where algorithms are given access to an oracle that predicts (e.g., based on modeling assumptions or on past data) the degrees of nodes in the graph. Within this model, we study the classic problem of online bipartite matching, and a natural greedy matching algorithm called MinPredictedDegree, which uses predictions of the degrees of offline nodes. For the bipartite version of a stochastic graph model due to Chung, Lu, and Vu where the expected values of the offline degrees are known and used as predictions, we show that MinPredictedDegree stochastically dominates any other online algorithm, i.e., it is optimal for graphs drawn from this model. Since the "symmetric" version of the model, where all online nodes are identical, is a special case of the well-studied "known i.i.d. model", it follows that the competitive ratio of MinPredictedDegree on such inputs is at least 0.7299. For the special case of graphs with power law degree distributions, we show that MinPredictedDegree frequently produces matchings almost as large as the true maximum matching on such graphs. We complement these results with an extensive empirical evaluation showing that MinPredictedDegree compares favorably to state-of-the-art online algorithms for online matching.

==> sections/experiments-arxiv.tex <==
In this section, we evaluate the empirical performance of MPD on real and synthetic data.
For each dataset, we report the empirical competitive ratio of MPD and a variety of baselines.
In each case, the empirical competitive ratio is the average, over 100 trials, of the ratios of the sizes of the matchings outputted by a given algorithm and the sizes of the maximum matching.
In addition to the average ratio, we report one standard deviation of the ratio across the trials.

\paragraph{Datasets}
We evaluate MPD on the following  datasets.
\begin{itemize}[leftmargin=*]
    \item \textbf{Oregon:} $9$ graphs\footnote{
        \label{foot-doublecover}The graphs in the Oregon and CAIDA datasets are made bipartite following the \emph{bipartite double cover} or \emph{duplicating method} used in prior work~\cite{ borodin2020experimental}. Given a graph $G=(V,E)$, the bipartite double cover of $G$ is the graph $G'=(U' \cup V', E')$ where $U'$ and $V'$ are copies of $V$ and there is an edge $\{u'_i, v'_j\} \in E'$ if and only if $\{v_i, v_j\} \in E$.
    }
    sampled over $3$ months representing a communication network of internet routers from the Stanford SNAP Repository~\cite{leskovec2014snap}. Each graph has $\sim 10k$ nodes on each side of the bipartition and $\sim 40k$ edges. For MPD, the offline degree predictor $\sigma: U \rightarrow \mathbb{R}$ is based on the first graph: if an offline node $u$ (i.e. a specific router) appeared in the first graph, $\sigma(u)$ is the degree of $u$ in that graph. If an offline node $u$ did not appear in the first graph, $\sigma(u) = 1$. 
    For each trial, the order of arrival of the online nodes is randomized.

    \item \textbf{CAIDA:} $122$ graphs\footnotemark[\value{footnote}] sampled approximately weekly over $4$ years representing a communication network of internet routers from the Stanford SNAP Repository~\cite{leskovec2014snap}.
    Each graph has $\sim 20k$ nodes on each side of the bipartition and $\sim 100k$ edges.
    The degree predictor is the same as for the Oregon dataset (for each year, the first graph of the year is used to form the predictor).
    As seen in Figure~\ref{fig-oracle-analysis} (see Appendix~\ref{appendix-experiments}), the degree distribution of the graphs for both the Oregon and Caida datasets are long-tailed and the error of the first graph predictor increases over time as the underlying graph evolves. 
    For each trial, the order of arrival of the online nodes is randomized.

    \item \textbf{Symmetric \GraphModel{} random graph:}
    We consider symmetric \GraphModel{} model where the expected offline degrees are distributed according to Zipf's Law, a popular power law distribution where $d_i = C \cdot i^{-\alpha}$~\cite{mitzenmacher2005probability}. 
    %\Piotr{This might be moved earlier, since we also use it for theory.}
    In our experiments, we set size $n=m=1000$, set $C=m/2$, and vary the exponent $\alpha$.
    %The performance of MPD on symmetric \GraphModel{} random graphs is further explored in Section~\ref{sec-analysis}.
    
    \item \textbf{Known i.i.d.:} 
    Finally, we compare MPD to algorithms for the known i.i.d.\ model, copying the methodology of Borodin et al.~\cite{borodin2020experimental} for synthetic power law graphs (Molloy Reed and Preferential Attachment) and real world graphs.
    In the Molloy Reed experiments, the type graph is sample from a family of random graphs with degrees distributed according to a power law with exponential cutoff.
    In the Preferential Attachment experiments, the type graph is formed by the preferential attachment model in which edges are added sequentially with edges between high degree nodes being more likely.
    The Real World graphs are comprised of a variety of graphs from the Network Repository~\cite{rossi2015networkrepository}. See Appendix~\ref{appendix-experiments} for more results on Real World graphs.
\end{itemize}

\paragraph{Baselines} We compare our algorithm to a variety of baseline algorithms.
\begin{itemize}[leftmargin=*]
    \item \textbf{Ranking} In all experiments, we compare to the classic, worst-case optimal Ranking algorithm~\cite{karp1990optimal}.
    
    \item \textbf{MinDegree} The MinDegree algorithm is a version of MPD with a perfect oracle, i.e. $\sigma(u)$ returns the true degree of $u$. In comparison with MPD, MinDegree shows the effect of prediction error on the performance of MPD.
    
    \item \textbf{Known i.i.d.\ baselines} For the experiments in the known i.i.d. case, we also compare to the baselines in the extensive empirical study of~\cite{borodin2020experimental}--see their paper for detailed descriptions of all algorithms. The code is distributed under the GPL license.
    % Most of these baselines rely on the type graph in order to do some preprocessing.
    Notably, the algorithms Category-Advice and 3-Pass are \emph{not} strictly online algorithms: they take multiple passes over the data, using some limited information from previous passes to make better decisions in the next pass.
    It should also be noted that BKPMinDegree is distinct from either the MPD or MinDegree algorithms we have described--it does not use the type graph but rather maintains and updates an estimate of the degree of the offline nodes throughout the runtime of the algorithm.
    
    Most known i.i.d.\ baselines are \emph{not} greedy--they do not always match an online node even if it has unmatched neighbors. \cite{borodin2020experimental} evaluate greedy augmentations of these algorithms (denoted by Algorithm(g)) which match to an arbitrary unmatched neighbor in these cases and generally show them to outperform their non-greedy counterparts. We additionally evaluate MPD augmented versions of these algorithms (denoted by Algorithm(MPD)) which applies the MPD rule in these cases using the expected degrees as predictions.
\end{itemize}

\begin{figure}[ht]
\begin{center}
% \centerline{\includegraphics[width=0.7\columnwidth]{plots/oregon1-neurips.pdf}}
\centerline{\includegraphics[width=0.4\columnwidth]{plots/oregon1-neurips.pdf}}
\caption{Comparison of empirical competitive ratios on the Oregon dataset. The first graph is used to form  predictions.}
\label{fig-oregon}
% \vspace{-0.25 in}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
% \centerline{\includegraphics[width=\columnwidth]{plots/caida.pdf}}
\centerline{\includegraphics[width=0.5\columnwidth]{plots/caida.pdf}}
\caption{Comparison of empirical competitive ratios on the CAIDA dataset. For each subfigure, the first graph of the year is used to form  predictions for the rest of the year.}
\label{fig-caida}
% \vspace{-0.25 in}
\end{center}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/zipfs_law_neurips.pdf}
    \caption{Comparison across Zipf's Law exponents.}
    \label{fig-zipf-comparison}
\end{subfigure}
\hspace{0.2 in}
\begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/zipfs_law_added_noise_subsample.pdf}
    \caption{Analysis of predictor noise (exponent $\alpha=1$).}
    \label{fig-zipf-noise}
\end{subfigure}
\caption{Comparison of empirical competitive ratios on symmetric \GraphModel{} random graphs with offline expected degrees following Zipf's Law with exponent $\alpha$. In (a), we vary $\alpha$ and MPD uses the expected degree as its predictor. In (b), the degree predictor is the offline degree in a random subgraph using a (varying) fraction of the online nodes.}
\label{fig-zipf}
% \vspace{-0.1 in}
\end{figure}

\begin{figure}[h!]
\begin{center}
\centerline{\includegraphics[width=0.5\columnwidth]{plots/borodinMolloyReed.pdf}}
\caption{Comparison of empirical competitive ratios on Molloy-Reed model. Algorithms depicted in gray are \emph{not} online algorithms (they use extra information or multiple passes). Algorithms in green make use of predicted degrees.}
\label{fig-molloyreed}
\vspace{-0.3 in}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\centerline{\includegraphics[width=0.5\columnwidth]{plots/borodinPreferentialAttachment.pdf}}
\caption{Comparison of empirical competitive ratios on Preferential Attachment graphs.}
\label{fig-preferentialattachment}
% \vspace{-0.25 in}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\centerline{\includegraphics[width=0.5\columnwidth]{plots/borodinRealWorld1.pdf}}
\caption{Comparison of empirical competitive ratios on Real World graphs. See Appendix~\ref{appendix-experiments} for more results.}
\label{fig-realworld}
% \vspace{-0.3 in}
\end{center}
\end{figure}
 
\paragraph{Results} Across the various datasets, MPD performs well compared to the baseline algorithms.
For the Oregon, CAIDA, and symmetric \GraphModel{} random graph datasets, MPD significantly outperforms Ranking, and for Oregon and CAIDA, the performance of the algorithm mildly declines as the degree predictions degrade.
For the known i.i.d.\ datasets, MPD often outperforms all \emph{online} baselines, despite making only limited use of the known i.i.d.\ model.
Additionally, augmenting the known i.i.d.\ algorithms with the (MPD) rule often improves their performance over both the base and the greedy (g) versions of the algorithms.
\begin{itemize}[leftmargin=*]
    \item \textbf{Oregon:} 
    On the Oregon dataset, MPD achieves a competitive ratio of $\sim 0.99$ across the graphs compared with competitive ratios ranging from $0.95$ to $0.97$ for Ranking.
    Compared with MinDegree, which uses knowledge of the true offline degrees, MPD's performance slowly degrades over time as the graphs become less similar to Graph $\# 1$ (see Figure~\ref{fig-oracle-analysis} in Appendix~\ref{appendix-experiments} for quantitative details).
    \item \textbf{CAIDA:} 
    Similarly to the Oregon dataset, on the CAIDA dataset, MPD does significantly better than Ranking, achieving competitive ratios almost always greater than $0.98$ compared to ratios around $0.95$, respectively.
    As the performance of the degree predictor degrades over time, the performance of MPD gradually declines (though it still significantly outperforms Ranking for both datasets).
    \item \textbf{Symmetric \GraphModel{} random graph:}
    For symmetric \GraphModel{} random graphs with offline expected degrees following Zipf's Law, MPD outperforms Ranking across a spectrum of exponents $\alpha$ ranging from $0.2$ to $2$.
    For exponents less than $0.5$ and greater than $1.5$, MPD achieves a competitive ratio close to $1$ (greater than $0.995$).
    All of the online algorithms have worse competitive ratios when the exponent is closer to one with MPD achieving a ratio of $\sim 0.93$ and Ranking achieving a ratio of $\sim 0.86$ when $\alpha=0.8$.
    Though MPD does worst at $\alpha=0.8$, it also achieves its greatest improvement over Ranking at this setting.
    %Using the equations in Section~\ref{sec-analysis}, in Figure~\ref{fig-analysis-zipf}, we see that for exponents other than $\alpha=1$, the competitive ratio of MPD improves as the size of the graph grows.
    
    In Figure~\ref{fig-zipf-noise}, we analyze the performance of MPD with a noisy degree predictor on Zipf's Law symmetric \GraphModel{} random graphs with exponent 1.
    To introduce noise, the degree predictor $\sigma(u)$ is given by the number of neighbors $u$ has with a random subset of the online nodes $V$.
    As we decrease the fraction of $V$ we subsample, thus increasing the variance of the predictor, the performance of MPD steadily declines.
    Even when the degree predictor only uses 10\% or even 1\% (the leftmost point on the graph) of the online nodes, it still outperforms Ranking.
    
    \item \textbf{Known i.i.d.:} Across all of the experiments in the known i.i.d.\ model, MPD is among the top online algorithms, and is often the best performing online algorithm (note the algorithms in gray are \emph{not} strictly online algorithms).
    Most of the algorithms (e.g.\ BahamiKapralov and ManshadiEtAl) rely heavily on the type graph, including precomputing an optimal matching on the type graph.
    By contrast, MPD only uses first-order information: it only looks at degrees and does not rely on any information about specific edges.
    Even so, in most cases, it outperforms all of the other online algorithms.
    Additionally, the (MPD) augmented versions of the known i.i.d.\ algorithms always beat the base algorithms and often beat the greedy (g) versions, indicating the potential of predicted degrees to be integrated with other algorithms.
    Note that while the standard deviations are quite wide (the known i.i.d.\ model is inherently stochastic), as the results are summarized over 100 trials, relatively small differences in the \emph{average} performance of these algorithms are statistically significant as the standard error is small.
\end{itemize}


